Training A Multi-stage Deep Classifier with Feedback Signals

Multi-Stage Classifier (MSC) - several classifiers working sequentially in an arranged order and classification decision is partially made at each step - is widely used in industrial applications for various resource limitation reasons. The classifiers of a multi-stage process are usually Neural Network (NN) models trained independently or in their inference order without considering the signals from the latter stages. Aimed at two-stage binary classification process, the most common type of MSC, we propose a novel training framework, named Feedback Training. The classifiers are trained in an order reverse to their actual working order, and the classifier at the later stage is used to guide the training of initial-stage classifier via a sample weighting method. We experimentally show the efficacy of our proposed approach, and its great superiority under the scenario of few-shot training.

==> TEX/related_work.tex <==

% [Will be merged into Intro Section, but hold it later.]

I.  Cascade and multi-stage process
multi-stage:

\cite{mendes2020multi} mitigated dual funnel problem by transferring knowledge from simpler early-stage neural networks to more complex networks in the latter stages. 



II. Resource limited solutions: small model  and multi-layer framework 



==> TEX/tables.tex <==
\begin{table}
\centering
\begin{tabular}{lcccccc}
\textbf{Language} & \textbf{pre\_recall} & \textbf{P} & \textbf{R} & \textbf{R\_e2e} & \textbf{F1\_e2e} & \textbf{Improv.} \\
    \midrule
    DE    & 0.671975 & 0.696429 & 0.924171 & 0.621019 & 0.656566 &  \\
          & 0.694268 & 0.721429 & 0.926606 & 0.643312 & 0.680135 & 3.59\% \\
    \midrule
    FR    & 0.594595 & 0.583026 & 0.897727 & 0.533784 & 0.557319 &  \\
          & 0.60473 & 0.596296 & 0.899441 & 0.543919 & 0.568905 & 2.08\% \\
    \midrule
    IT    & 0.615385 & 0.653846 & 0.929688 & 0.572115 & 0.610256 &  \\
          & 0.697115 & 0.658537 & 0.931034 & 0.649038 & 0.653753 & 7.13\% \\
    \midrule
    PT    & 0.716814 & 0.697674 & 0.925926 & 0.663717 & 0.680272 &  \\
          & 0.730088 & 0.701835 & 0.927273 & 0.676991 & 0.689189 & 1.31\% \\
    \bottomrule
    \end{tabular}
  \caption{Feedback training result on Task Extraction for different languages. In each group, the first line denotes the result of independent training while the second line is for feedback training, all the following table using the same setting of display for experiment results. Besides the main models for all languages share a same multi-lingual model.}
  \label{tab:accents}
\end{table}

\begin{table}
\centering
\begin{tabular}{lcccccc}
\textbf{Model} & \textbf{pre\_recall} & \textbf{P} & \textbf{R} & \textbf{R\_e2e} & \textbf{F1\_e2e} & \textbf{Improv.}\\
    \midrule
    4 Layer &  0.724225 & 0.667391 & 0.500349 & 0.362365 & 0.469702 &  \\
          &  0.739387 & 0.663076 & 0.505014 & 0.373400 & 0.477759 & 1.72\% \\
    \midrule
    8 Layer &  0.724225 & 0.720144 & 0.46569 & 0.337264 & 0.459385 &  \\
          &  0.739387 & 0.714086 & 0.466727 & 0.345092 & 0.465315 & 1.29\% \\
    \midrule
    12 Layer &  0.724225 & 0.700945 & 0.448709 & 0.324966 & 0.444061 &  \\
          &  0.739387 & 0.696756 & 0.450319 & 0.332960 & 0.450594 & 1.47\% \\
    \bottomrule
    \end{tabular}%
 \caption{Feedback Training vs different size of main model, pass rate for all were set to be 0.3.}
%   \label{tab:accents}
\end{table}


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}
  \centering
\begin{tabular}{lcccccc}
\textbf{Pass Rate} & \textbf{pre\_recall} & \textbf{P} & \textbf{R} & \textbf{R\_e2e} & \textbf{F1\_e2e} & \textbf{Improv.} \\
    \midrule
    0.2   &  0.616071 & 0.705948 & 0.515997 & 0.317891 & 0.438378 &  \\
          &  0.62938 & 0.704471 & 0.518737 & 0.326482 & 0.446184 & 1.78\% \\
    \midrule
    0.3   &  0.724225 & 0.700945 & 0.448709 & 0.324966 & 0.444061 &  \\
          &  0.739387 & 0.696756 & 0.450319 & 0.332960 & 0.450594 & 1.47\% \\
    \midrule
    0.4   &  0.803403 & 0.698748 & 0.40952 & 0.329009 & 0.447371 &  \\
          &  0.791442 & 0.692335 & 0.42103 & 0.333221 & 0.449903 & 0.57\% \\
    \midrule
    0.5   &  0.87062 & 0.695285 & 0.382353 & 0.332884 & 0.450216 &  \\
          &  0.885782 & 0.693209 & 0.382465 & 0.338780 & 0.455132 & 1.09\% \\
    \bottomrule
    \end{tabular}
  \caption{Feedback Training vs different pass rate, all of the main model used 12 layer transformer.}
%   \label{tab:accents}
\end{table}


\begin{table}
  \centering
    \begin{tabular}{lcccccc}
    \textbf{DataSet} &  \textbf{pre\_recall} & \textbf{P} & \textbf{R} & \textbf{R\_e2e} & \textbf{F1\_e2e} & \textbf{Improv.} \\
    \midrule
    1\% Organic &  0.4797844 & 0.7428243 & 0.454992968 & 0.2182985 & 0.3374333 & - \\
    1\% Organic &  0.6415094 & 0.717477 & 0.474232774 & 0.3042248 & 0.4272759 & 26.63\% \\
    \midrule
    1\% Organic+Aug & 0.5921496 & 0.7174199 & 0.465414176 & 0.2755948 & 0.3982161 & - \\
    1\% Organic+Aug & 0.7265836 & 0.6982507 & 0.468688845 & 0.3405416 & 0.4578074 & 14.96\% \\
    \midrule
    2\% Organic & 0.5158356 & 0.7355623 & 0.474199869 & 0.2446092 & 0.3671302 & - \\
    2\% Organic & 0.666779 & 0.7117552 & 0.485580884 & 0.3237751 & 0.4450833 & 21.23\% \\
    \midrule
    5\% Organic & 0.5675539 & 0.7210046 & 0.46868507 & 0.266004 & 0.3886291 & - \\
    5\% Organic & 0.6686321 & 0.7075579 & 0.469387755 & 0.3138477 & 0.4348232 & 11.89\% \\
    \midrule
    10\% Organic & 0.6010782 & 0.7191601 & 0.460762332 & 0.2769542 & 0.3999027 & - \\
    10\% Organic & 0.7179919 & 0.7019868 & 0.466503667 & 0.3349459 & 0.453506 & 13.40\% \\
    \midrule
    50\% Organic & 0.7179919 & 0.7025316 & 0.459571359 & 0.3299685 & 0.449033 & - \\
    50\% Organic & 0.7350067 & 0.7006927 & 0.456857618 & 0.3357934 & 0.4540109 & 1.11\% \\
    \bottomrule
    \end{tabular}
\caption{Using a proportion of data to train preclassifer. It shows that Feedback Learning gains a very large improvement on the E2E performance in small dataset and acquired the same performance of whole data training by using only 10\% of the data and could reduce the proportion to 1\% when data augmentation is adopted, which shows its strong ability of data selection.}
%   \label{tab:accents}
\end{table}


\begin{table}[htbp]
  \centering
    \begin{tabular}{lcccccc}
    \toprule
    \textbf{DataSet} & \textbf{pre\_recall} & \textbf{P} & \textbf{R} & \textbf{R\_e2e} & \textbf{F1\_e2e} & \textbf{Improv.} \\
    \midrule
    5\% Organic & 0.5675539 & 0.6675933 & 0.4989611 & 0.2831873 & 0.3976816 &  \\
    5\% Organic & 0.7031671 & 0.6560157 & 0.5065458 & 0.3561864 & 0.4616941 & 16.10\% \\
    \midrule
    10\% Organic & 0.6010782 & 0.6720993 & 0.485426 & 0.291779 & 0.4069071 &  \\
    10\% Organic & 0.7147911 & 0.6574283 & 0.5011054 & 0.3581857 & 0.4637222 & 13.96\% \\
    \midrule
    25\% Organic & 0.652965 & 0.7289916 & 0.4476264 & 0.2922844 & 0.4172679 &  \\
    25\% Organic & 0.7351752 & 0.717475 & 0.4432818 & 0.3258898 & 0.4481995 & 7.41\% \\
    \midrule
    50\% Organic & 0.7179919 & 0.762704 & 0.3984413 & 0.2860776 & 0.4160877 &  \\
    50\% Organic & 0.7348383 & 0.760274 & 0.3958631 & 0.2908953 & 0.4207888 & 1.13\% \\
    \bottomrule
    \end{tabular}%
\caption{Training the whole pipeline using different proportion of data}
% \label{tab:accents}%
\end{table}%


\begin{table}
\centering
\begin{tabular}{lcccccc}
\textbf{Setting} & \textbf{pre\_recall} & \textbf{P} & \textbf{R} & \textbf{R\_e2e} & \textbf{F1\_e2e} & \textbf{Improv.} \\
\midrule
Baseline & 0.724225 & 0.700945 & 0.448709 & 0.324966 & 0.444061 &  \\
No ablation & 0.739387 & 0.696756 & 0.450319 & 0.33296 & 0.450594 & 1.47\% \\
w\_neg\_min=0 & 0.739387 & 0.696756 & 0.450319 & 0.33296 & 0.450594 & 1.47\% \\
w\_max=2 & 0.727931 & 0.700945 & 0.448709 & 0.326629 & 0.445611 & 0.35\% \\
w\_neg\_min=0,w\_max=2 & 0.727931 & 0.700287 & 0.45162 & 0.328749 & 0.447445 & 0.76\% \\
\bottomrule
\end{tabular}
\caption{Ablation studies of $w_{neg\_min}$ and $w_{max}$ in weighting function, pass rate=0.3.}
% \label{tab:accents}
\end{table}



\begin{figure}[htb]
    \centering
        \subfigure[]
            {
                \begin{minipage}[htbp]{1.0\linewidth}
                \centering
                \setlength{\abovecaptionskip}{0.cm}
                \includegraphics[width=0.9\textwidth]{Figures/feedback.png}
                \label{fig:a}
                \end{minipage}
            }\hspace{-30mm}
\caption{(a) Matching model architecture with symmetric loss and TLM/MLM cross-entropy loss. 
(b) Multi-task continual training loop for EUR->NAM->LRL clusters.
}
\label{fig1}
\end{figure}
